MIGE: Mutually Enhanced Multimodal Instruction-Based Image Generation and Editing

Despite significant progress in diffusion-based image generation, subject-driven generation and instruction-based editing remain challenging. Existing methods typically treat them separately, struggling with limited high-quality data and poor generalization. However, both tasks require capturing complex visual variations while maintaining consistency between inputs and outputs. Inspired by this, we propose MIGE, a unified framework that standardizes task representations using multimodal instructions. It first treats subject-driven generation as creation on a blank canvas and instruction-based editing as modification of an existing image, establishing a shared input-output formulation, then introduces a novel multimodal encoder that maps free-form multimodal instructions into a unified vision-language space, integrating visual and semantic features through a feature fusion mechanism. This unification enables joint training of both tasks, providing two key advantages: (1) Cross-Task Enhancement: by leveraging shared visual and semantic representations, joint training improves instruction adherence and visual consistency in both subject-driven generation and instruction-based editing. (2) Generalization: learning in a unified format facilitates cross-task knowledge transfer, enabling MIGE to generalize to novel compositional tasks, including instruction-based subject-driven editing. Experiments show that MIGE excels in both subject-driven generation and instruction-based editing while setting a SOTA in the new task of instruction-based subject-driven editing. Code and model have been publicly available at https://github.com/Eureka-Maggie/MIGE.

==> sections/framework.tex <==
\subsection{Task Unification}
%Subject-driven generation and instruction-based editing suffer from limited data and poor generalization when modeled independently, largely due to the complex interplay between subject information and textual instructions. Unifying these tasks leverages their complementary nature, as both require coordinating multimodal instructions. A unified framework optimizes subject recognition and text-guided processing, improving the model’s ability to capture and preserve subject indentity. This approach mitigates the limitations of single-task methods, enhancing subject consistency with greater precision and naturalness. 
%We achieve task unification through the combination of unified representation and a consistent model design, as illustrated in Figure \ref{fig:format}.

Current methods treat subject-driven generation and instruction-based image editing separately, hindering performance due to data limitations and poor generalization. Since both aim to preserve visual consistency while incorporating instructed changes, unifying them allows mutual improvement.  Joint training on diverse data enhances subject preservation and instruction following beyond the capabilities of individual task-specific models.

Therefore, we propose \method to unify the two tasks for joint training. By using multimodal instructions as a unified task representation, it supports flexible combinations and provides multimodal guidance. Additionally, we use conditional input to structurally unify the tasks, enhancing visual consistency. Their combination not only provides rich visual and instructional information but also naturally represents different tasks. We demonstrate the input-output format of \method in Figure \ref{fig:format}.

% while the interleaved vision-language format provides rich multimodal information
% supporting diverse combinations of tasks and instructions
%Our approach combines conditional input and multimodal instruction to ensure subject fidelity and precise edits. Conditional input provides clear guidance, maintaining input-output coherence, while multimodal instruction enhances cross-modal understanding, offering rich information for modifications. This integrated design improves flexibility and scalability, boosting performance across diverse editing and generation tasks.

%In subject-driven image generation, the model must ensure subject consistency across varied scenes and follow textual descriptions. In instruction-based image editing, the model needs to modify the subject in an existing image while preserving overall image integrity.
%By unifying these tasks, we can leverage shared model architecture and training strategies to enhance both tasks, improving generalization and enabling more flexible, multi-controllable generation.
%这两个任务在单一建模时都面临数据不足和泛化性差的问题，根本原因在于如何有效识别和保持视觉特征中的主体一致性，同时处理主体信息与文本指令之间复杂的关系。在subject-driven image generation任务中，生成模型需要确保在多变的场景下保持主体一致性，并准确响应文本描述。而在instruction-based image editing任务中，模型则需要在已有图像的基础上对主体进行修改，同时确保主体特征不被破坏。这两个任务的共同挑战在于，如何准确理解并维持主体信息，同时处理文本指令与视觉内容之间的关系。统一框架可以共同优化主体识别和文本引导的处理，使得模型在多模态指令下能够更准确地捕捉和保持主体信息，从而克服传统方法在执行单一任务时的局限性。这种协同训练不仅提高了任务之间的共性处理能力，也使得两类任务在处理主体一致性时更加精确、自然。


\paragraph{Unified Multimodal Instruction}
To enable joint training across multiple tasks, a unified task representation is essential. We introduce multimodal instructions composed of interleaved images and text, which provide both visual references and textual guidance for various controllable generation tasks. As shown in Figure \ref{fig:format}, ``<imagehere>'' serves as a placeholder, sequentially replaced by input images, which can be the reference subject or the entire scene, complementing the semantics to form interleaved expressions. This unified approach effectively accommodates subject-driven generation and instruction-based editing while remaining extensible to the more complex combination task. 

\paragraph{Unified Conditional Input}
We adopt a conditional input design to unify tasks structurally, ensuring clear task distinction while enabling shared capabilities. By concatenating different conditions, we differentiate initial generation states and capture task-specific nuances, enhancing execution accuracy. As shown in Figure \ref{fig:format}, for instruction-based editing, we concatenate the VAE-encoded source image with the noise tensor, guiding generation based on the given image. For subject-driven generation, we use an all-zero tensor akin to a blank canvas, prompting the model to generate freely while preserving specified visual features.
This design effectively captures the differences between the two tasks while ensuring input-output consistency in editing. Moreover, structuring tasks within a unified framework allows the model to leverage shared capabilities and easily extend to new tasks.

%为什么这么设计： 自然地区分不同任务，任务间共享能力，同时保留独特性，学习到任务之间的微妙区别，提高任务执行的准确性 所以To unify tasks structurally, we design a conditional input. As shown in Figure \ref{fig:format}, we distinguish tasks by concatenating different conditions to represent distinct initial generation states. In diverse instruction-based editing tasks, we concatenate the VAE-encoded source image to the noise tensor along the channel dimension, guiding the model to generate based on the given image. In subject-driven generation, we concatenate an all-zero tensor of the same dimension, akin to a blank canvas, indicating the model to freely create based on text descriptions while preserving the visual attributes specified in the multimodal instruction. // 好处：This representation effectively captures the differences between the two tasks while ensuring high consistency between input and output in editing tasks. 对 精确编辑、保持局部细节 以及 减少无关区域的改变 更加有效，提高推理稳定性：减少任务混淆，


